Quantum State Assignment Flows

This paper introduces assignment flows for density matrices as state spaces for representing and analyzing data associated with vertices of an underlying weighted graph. Determining an assignment flow by geometric integration of the defining dynamical system causes an interaction of the non-commuting states across the graph, and the assignment of a pure (rank-one) state to each vertex after convergence. Adopting the Riemannian Bogoliubov-Kubo-Mori metric from information geometry leads to closed-form local expressions which can be computed efficiently and implemented in a fine-grained parallel manner. Restriction to the submanifold of commuting density matrices recovers the assignment flows for categorial probability distributions, which merely assign labels from a finite set to each data point. As shown for these flows in our prior work, the novel class of quantum state assignment flows can also be characterized as Riemannian gradient flows with respect to a non-local non-convex potential, after proper reparametrization and under mild conditions on the underlying weight function. This weight function generates the parameters of the layers of a neural network, corresponding to and generated by each step of the geometric integration scheme. Numerical results indicates and illustrate the potential of the novel approach for data representation and analysis, including the representation of correlations of data across the graph by entanglement and tensorization.

==> TexInput/Contributions.tex <==
%!TEX root =  ../QSAF2023.tex
\subsection{Riemannian Gradient, Replicator Operator and Further Mappings}\label{sec:grad-R-density}


As described in \cite{Hasegawa:1993vv}, the general $\alpha-$Divergence can be written as
\begin{align}
	g^{(\alpha)}(X,Y) = \tr \left( X \ell^{(\alpha)}(\rho), Y \ell^{(\alpha)}(\rho)\right)
\end{align}
with 
\begin{equation}
	\ell^{(\alpha)} = \begin{cases} \frac{2}{1-\alpha} \rho^{\frac{1-\alpha}{2}} \quad & (\alpha \neq 1) \\ \log(\rho) \quad & (\alpha = 1) \end{cases}.
\end{equation}
This yields for $\alpha =1$ the standard





\begin{proposition}\label{prop:grad-Dc}
	Let $f\colon\mc{D}_{c}\to\R$ be a smooth function defined on the manifold \eqref{eq:def-mcDc}. Then its Riemannian gradient with respect to the BKM-metric \eqref{eq:Bogoliubov} is given by
	\begin{equation}\label{eq:grad-Dc}
	\ggrad_{\rho}f = \mb{T}_{\rho}^{-1}[\partial f] - \la \rho, \partial f \ra\rho,
	\end{equation}
	where $\mb{T}_{\rho}^{-1}$ is given by \eqref{eq:def-mcT-inverse} and $\partial f$ is the ordinary gradient with respect to the Euclidean structure of the ambient space $\R^{c\times c}$.
	\end{proposition}
	%
	\begin{proof}
		Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
	\end{proof}
	%
	


	\vspace{0.25cm}
	Comparing the result \eqref{eq:grad-Dc} with \eqref{eq:grad-R-simplex} motivates to define the
	\begin{equation}\label{eq:def-Rrho}
	R_{\rho}\colon\mc{H}_{c}\to\mc{H}_{c;0},\qquad
	R_{\rho}[X] := \mb{T}_{\rho}^{-1}[X]-\la \rho,X\ra\rho,\qquad\rho\in\mc{D}_{c}
	\qquad\qquad(\text{replicator map})
	\end{equation}
	The following lemma shows that the properties \eqref{eq:Rp-Pi0} extend to \eqref{eq:def-Rrho}.
	%
	\begin{lemma}\label{lem:repl-proj-rho-commute}
	Let $\Pi_{c;0}$ denote the orthogonal projection \eqref{eq:def-Pic0}. Then the replicator map \eqref{eq:def-Rrho} satisfies
	\begin{equation}\label{eq:Pic0-Rrho-commute}
	\Pi_{c;0}\circ R_{\rho}
	= R_{\rho}\circ \Pi_{c;0} 
	= R_{\rho},
	\quad\forall\rho\in\mc{D}_{c}.
	\end{equation}
	\end{lemma}
	%
	%
	
	\vspace{0.25cm}
Next, using the tangent space $\mc{H}_{c;0}$, we define a parametrization of the manifold $\mc{D}_{c}$ in terms of the mapping
	\begin{subequations}\label{eq:def-Gamma}
	\begin{align}\label{eq:def-Gamma-a}
	\Gamma\colon\mc{H}_{c;0}\to\mc{D}_{c},\qquad
	\Gamma(X) 
	&:= \frac{\expm(X)}{\tr\expm(X)}
	= \expm\big(X-\psi(X)I\big),
	\intertext{where}\label{eq:def-psi-Gamma}
	\psi(X) &:= \log\big(\tr\expm(X)\big).
	\end{align}
	\end{subequations}
	The following lemma and proposition explain why the domain of $\Gamma$ extends to $\R^{c\times c}$ without change.
	%
	\begin{lemma}\label{lem:Gamma-Pi0}
	Let $Z\in\R^{c\times c}$. Then the extension to $\R^{c\times c}$ of the mapping $\Gamma$ defined by \eqref{eq:def-Gamma} satisfies
	\begin{equation}\label{eq:Gamma-Pi0}
	\Gamma(Z) = \Gamma(\Pi_{c;0}[Z]).
	\end{equation}
	\end{lemma}
	%
	\begin{proof}
		Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
	\end{proof}
	%

	\begin{proposition}\label{prop:Gamma-invertible}
	The map $\Gamma$ defined by \eqref{eq:def-Gamma} is bijective with inverse
	\begin{equation}\label{eq:def-Gamma-1}
	\Gamma^{-1}\colon\mc{D}_{c}\to\mc{H}_{c;0},\qquad
	\Gamma^{-1}(\rho) = \Pi_{c;0}[\logm\rho].
	\end{equation}
	\end{proposition}
	%
	\begin{proof}
		Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
	\end{proof}





\begin{proposition}\label{prop:grad-Dc}
Let $f\colon\mc{D}_{c}\to\R$ be a smooth function defined on the manifold \eqref{eq:def-mcDc}. Then its Riemannian gradient with respect to the BKM-metric \eqref{eq:Bogoliubov} is given by
\begin{equation}\label{eq:grad-Dc}
\ggrad_{\rho}f = \mb{T}_{\rho}^{-1}[\partial f] - \la \rho, \partial f \ra\rho,
\end{equation}
where $\mb{T}_{\rho}^{-1}$ is given by \eqref{eq:def-mcT-inverse} and $\partial f$ is the ordinary gradient with respect to the Euclidean structure of the ambient space $\R^{c\times c}$.
\end{proposition}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
%
%

\vspace{0.25cm}
Comparing the result \eqref{eq:grad-Dc} with \eqref{eq:grad-R-simplex} motivates to define the
\begin{equation}\label{eq:def-Rrho}
R_{\rho}\colon\mc{H}_{c}\to\mc{H}_{c;0},\qquad
R_{\rho}[X] := \mb{T}_{\rho}^{-1}[X]-\la \rho,X\ra\rho,\qquad\rho\in\mc{D}_{c}
\qquad\qquad(\text{replicator map})
\end{equation}
The following lemma shows that the properties \eqref{eq:Rp-Pi0} extend to \eqref{eq:def-Rrho}.
%
\begin{lemma}\label{lem:repl-proj-rho-commute}
Let $\Pi_{c;0}$ denote the orthogonal projection \eqref{eq:def-Pic0}. Then the replicator map \eqref{eq:def-Rrho} satisfies
\begin{equation}\label{eq:Pic0-Rrho-commute}
\Pi_{c;0}\circ R_{\rho}
= R_{\rho}\circ \Pi_{c;0} 
= R_{\rho},
\quad\forall\rho\in\mc{D}_{c}.
\end{equation}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%

\vspace{0.25cm}
Next, using the tangent space $\mc{H}_{c;0}$, we define a parametrization of the manifold $\mc{D}_{c}$ in terms of the mapping
\begin{subequations}\label{eq:def-Gamma}
\begin{align}\label{eq:def-Gamma-a}
\Gamma\colon\mc{H}_{c;0}\to\mc{D}_{c},\qquad
\Gamma(X) 
&:= \frac{\expm(X)}{\tr\expm(X)}
= \expm\big(X-\psi(X)I\big),
\intertext{where}\label{eq:def-psi-Gamma}
\psi(X) &:= \log\big(\tr\expm(X)\big).
\end{align}
\end{subequations}
The following lemma and proposition explain why the domain of $\Gamma$ extends to $\R^{c\times c}$ without change.
%
\begin{lemma}\label{lem:Gamma-Pi0}
Let $Z\in\R^{c\times c}$. Then the extension to $\R^{c\times c}$ of the mapping $\Gamma$ defined by \eqref{eq:def-Gamma} satisfies
\begin{equation}\label{eq:Gamma-Pi0}
\Gamma(Z) = \Gamma(\Pi_{c;0}[Z]).
\end{equation}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%

\begin{proposition}\label{prop:Gamma_inverse}
The map $\Gamma$ defined by \eqref{eq:def-Gamma} is bijective with inverse
\begin{equation}\label{eq:def-Gamma-1}
\Gamma^{-1}\colon\mc{D}_{c}\to\mc{H}_{c;0},\qquad
\Gamma^{-1}(\rho) = \Pi_{c;0}[\logm\rho].
\end{equation}
\end{proposition}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
The following lemma provides the diffentials of the mappings $\Gamma$ and $\Gamma^{-1}$.
%
\begin{lemma}\label{lem:dGamma-1}
Let $H, X\in\mc{H}_{c;0}$ with $\Gamma(H)=\rho$ and $Y\in T\mc{H}_{c;0}\cong\mc{H}_{c;0}$. Then
\begin{subequations}
\begin{align}\label{eq:dGamma-H}
d\Gamma(H)[Y] 
&= \mb{T}_{\rho}^{-1}\big[Y-\la\rho,Y\ra I\big],\qquad
\rho=\Gamma(H),
\\ \label{eq:dGamma-1}
d\Gamma^{-1}(\rho)[X] 
&= \Pi_{c;0}\circ\mb{T}_{\rho}[X].
\end{align}
\end{subequations}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
We finally compute a closed-form expression of the e-geodesic, i.e.~the geodesic resp.~exponential map induced by the e-connection on the manifold $(\mc{D}_{c},g)$.
%
\begin{proposition}\label{prop:e-geodesic}
The e-geodesic emanating at $\rho\in\mc{D}_{c}$ in the direction $X\in\mc{H}_{c;0}$ and the corresponding exponential map are given by
\begin{subequations}\label{eq:e-geodesic}
\begin{align}
\gamma_{\rho,X}^{(e)}(t)
&:= \Exp_{\rho}^{(e)}(t X),\quad t\geq 0
\label{eq:e-geodesic-a} \\ \label{eq:def-Exp-rho-e}
\Exp_{\rho}^{(e)}(X)
&:= \Gamma\big(\Gamma^{-1}(\rho)+d\Gamma^{-1}(\rho)[X]\big)
\\ \label{eq:def-Exp-rho-e-b}
&= \Gamma\big(\Gamma^{-1}(\rho)+\Pi_{c;0}\circ\mb{T}_{\rho}[X]\big).
\end{align}
\end{subequations}
\end{proposition}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}

%
\begin{corollary}\label{cor:Exp-1}
The inverse of the exponential mapping \eqref{eq:e-geodesic} is given by
\begin{equation}\label{eq:Exp-1}
\big(\Exp_{\rho}^{(e)}\big)^{-1}\colon\mc{D}_{c}\to\mc{H}_{c;0},\qquad
\big(\Exp_{\rho}^{(e)}\big)^{-1}(\mu)
= d\Gamma\big(\Gamma^{-1}(\rho)\big)\big[\Gamma^{-1}(\mu)-\Gamma^{-1}(\rho)\big].
\end{equation}
\end{corollary}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
Analogous to \eqref{eq:def_exp_standard_af}, we define the mapping $\exp_{\rho}$, where both the subscript and the argument disambiguate how the symbol `$\exp$' is used.
%




\begin{lemma}\label{lem:exp-rho}
The mapping defined using \eqref{eq:def-Exp-rho-e} and \eqref{eq:def-Rrho} as
\begin{subequations}\label{eq:def-exp-rho}
\begin{align}\label{eq:def-exp-rho-a}
\exp_{\rho}\colon\mc{H}_{0;c}\to\mc{D}_{c},\qquad
\exp_{\rho}(X) 
&:= \Exp_{\rho}^{(e)}\circ R_{\rho}[X],\qquad
\rho\in\mc{D}_{c}
\intertext{has the explicit form}\label{eq:def-exp-rho-b}
\exp_{\rho}(X) 
&= \Gamma \big( \Gamma^{-1}(\rho) + X \big).
\end{align}
\end{subequations}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
The following Lemma provides the explicit form of the differential of the mapping \eqref{eq:def-exp-rho-b} which resembles the corresponding formula \eqref{eq:dexp-p} of the assignment flow.
%
\begin{lemma}\label{lem:dexp-rho}
The differential of the mapping \eqref{eq:def-exp-rho} reads with $\rho\in\mc{D}_{c}$, $X\in\mc{H}_{c;0}$ and $Y\in T\mc{H}_{c;0}\cong\mc{H}_{c;0}$
\begin{equation}\label{eq:dexp-rho}
d\exp_{\rho}(X)[Y]
= R_{\exp_{\rho}(X)}[Y].
\end{equation}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
\begin{remark}\label{rem:similarity-to-AF-1}
Since \eqref{eq:dexp-rho} resembles \eqref{eq:dexp-p}, one may wonder about the connection of \eqref{eq:def-exp-rho-b} and \eqref{eq:def_exp_standard_af}. In view of \eqref{eq:def-Gamma-a}, we define
\begin{equation}
\gamma\colon T_{c;0}\to\mc{S}_{c},\qquad
\gamma(v) := \frac{e^{v}}{\la\eins,e^{v}\ra}
= \exp_{\eins_{\mc{S}_{c}}}(v)
\end{equation}
and compute with the expression for its inverse (cf.~\cite{savarino2021continuous})
\begin{subequations}
\begin{align}
\gamma^{-1}(p) 
&= \pi_{c;0}\log\frac{p}{\eins_{\mc{S}_{c}}}
= \pi_{c;0}(\log p-\log\eins_{\mc{S}_{c}})
= \pi_{c;0}\log p
\\
&\overset{\eqref{eq:def-Pi0-p}}{=} 
\log p - \la \eins_{\mc{S}_{c}},\log p\ra\eins_{c}
\end{align}
\end{subequations}
which resembles \eqref{eq:def-Gamma-1}. Moreover, in view of \eqref{eq:def-exp-rho-b}, the analogous expression using $\gamma$ instead of $\Gamma$ reads
\begin{subequations}
\begin{align}
\gamma\big(\gamma^{-1}(p)+v\big)
&= \frac{e^{\pi_{c;0}\log p + v}}{\la\eins,e^{\pi_{c;0}\log p + v}\ra}
= \frac{\la\eins_{\mc{S}_{c}},\log p\ra p\cdot e^{v}}{\la \la\eins_{\mc{S}_{c}},\log p\ra p,e^{v}\ra}
= \frac{p\cdot e^{v}}{\la p,e^{v}\ra}
\\
&= \exp_{p}(v).
\end{align}
\end{subequations}
\end{remark}
%




\subsection{Single-Vertex Density Matrix Assignment Flow}\label{sec:single-vertex-DAF}

We generalize the single vertex assignment flow equation \eqref{eq:single-vertex-AF} to the manifold $\mc{D}_{c}$ \eqref{eq:def-mcDc}. 

Defining in view of \eqref{eq:def-LpD} the \textit{likelihood matrix}
\begin{equation}\label{eq:def-L-rho-D}
L_{\rho}\colon\mc{H}_{c}\to\mc{D}_{c},\qquad
L_{\rho}(D) := \exp_{\rho}(-\Pi_{c;0}[D]),\qquad
\rho\in\mc{D}_{c},
\end{equation}
the corresponding \textit{single vertex density matrix assignment flow} equation reads
\begin{subequations}\label{eq:single-vertex-matrix-flow}
\begin{align}
\dot\rho &= R_{\rho}[L_{\rho}(D)]
\\ \label{eq:single-vertex-matrix-flow-b}
&\overset{\eqref{eq:def-Rrho}}{=} 
\mb{T}_{\rho}^{-1}[L_{\rho}(D)] - \la\rho,L_{\rho}(D)\ra\rho,\qquad
\rho(0)=\eins_{\mc{D}_{c}}=\Diag(\eins_{\mc{S}_{c}}).
\end{align}
\end{subequations}
Our goal is to prove Proposition \ref{prop:single-vertex-matrix-flow} below after a preparatory Lemma.
%
\begin{lemma}\label{lem:rho-LD-diagonalized}
Assume 
\begin{equation}\label{eq:lem-rho-LD-decomposition}
D=Q\Lambda_{D}Q^{\T}\in\mc{H}_{c} 
\qquad\text{and}\qquad 
\rho=Q\Lambda_{\rho}Q^{\T}\in\mc{D}_{c}
\end{equation}
can be simultaneously diagonalized with $Q\in\LG{O}(d)$, $\Lambda_{D}=\Diag(\lambda_{D})$, $\Lambda_{\rho}=\Diag(\lambda_{\rho})$ and $\lambda_{\rho}\in\mc{S}_{c}$ since $\tr\rho=1$. Then
\begin{equation}
L_{\rho}(D) = Q \Diag\big(\exp_{\lambda_{\rho}}(-\lambda_{D})\big) Q^{\T}.
\end{equation}
\end{lemma}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%
%
%
\begin{proposition}\label{prop:single-vertex-matrix-flow}
Let $D = Q\Lambda_{D}Q^{\T}$ be the spectral decomposition of $D$ with eigenvalues $\lambda_{1}\geq\dotsb\geq\lambda_{c}$ and orthonormal eigenvectors $Q = (q_{1},\dotsc,q_{c})$. Assume the minimal eigenvalue $\lambda_{c}$ is unique. Then the solution $\rho(t)$ to \eqref{eq:single-vertex-matrix-flow} satisfies
\begin{equation}
\lim_{t\to\infty}\rho(t) = \Pi_{q_{c}} := q_{c}q_{c}^{\T}.
\end{equation}
\end{proposition}
%
\begin{proof}
	Proof in Appendix \ref{sec:appendix-quantum-state-assignment-flow}.
\end{proof}
%





